Support Recovery of Periodic Mixtures with Nested Periodic Dictionaries

Periodic signals composed of periodic mixtures admit sparse representations in nested periodic dictionaries (NPDs). Therefore, their underlying hidden periods can be estimated by recovering the exact support of said representations. In this paper, support recovery guarantees of such signals are derived both in noise-free and noisy settings. While exact recovery conditions have been studied in the theory of compressive sensing, existing conditions fall short of yielding meaningful achievability regions in the context of periodic signals with sparse representations in NPDs, in part since existing bounds do not capture structures intrinsic to these dictionaries. We leverage known properties of NPDs to derive several conditions for exact sparse recovery of periodic mixtures in the noise-free setting. These conditions rest on newly introduced notions of nested periodic coherence and restricted coherence, which can be efficiently computed. In the presence of noise, we obtain improved conditions for recovering the exact support set of the sparse representation of the periodic mixture via orthogonal matching pursuit based on the introduced notions of coherence. The theoretical findings are corroborated using numerical experiments for different families of NPDs. Our results show significant improvement over generic recovery bounds as the conditions hold over a larger range of sparsity levels.

==> Background/Nested_Periodic_Dictionary/Ramanujan_subspaces.tex <==
 \subsection{Ramanujan subspaces}
\label{subsec:Ramanujan_subspaces}
The Ramanujan subspace $\mathcal{S}_q$ is defined as the column space of the periodically extended version of the matrix $\bC_q$ in \eqref{eq:C_q}.
Two compelling features of the Ramanujan subspace can be described as follow.
\begin{itemize}
    \item The dimension of $\mathcal{S}_p$ is $\phi\left(p\right)$ \cite{tenneti2015nested},\cite{vaidyanathan2014ramanujanI}, that is known as the Euler structure
    \cite{tenneti2016unified}.
    \item For the signals that are in the Ramanujan subspace and constitute the mixture in \eqref{eq:mixture_definition}, the period of the mixture is exactly the least common multiplier (LCM) of the hidden periods and not a divisor of the LCM. This is known as the LCM property \cite{tenneti2016unified}.
\end{itemize}
It is important to note that in \cite{tenneti2016unified}, Tenneti and Vaidyanathan defined the broader nested periodic subspaces (NPSs), that are the span of $\bC_{p}$'s, the submatrices that construct a NPM. NPSs enjoy the LCM property. However, the Ramanujan subspaces are considered a special case of NPSs, because of the orthogonality of the subspaces, i.e., $\mathcal{S}_i \perp \mathcal{S}_j$. In other words, whenever the orthogonality of the NPSs preserved then those NPSs are the Ramanujan subspaces.


==> Background/Nested_Periodic_Dictionary/minimum_length.tex <==
Given the Farey dictionary as an instance of NPDs, it was shown in \cite{tenneti2018minimum} that to recover the exact support set for a periodic mixture consisting of $m$ hidden periods as in \eqref{eq:mixture_definition} with hidden periods in $\mathbb{P}$, it is both necessary and sufficient that
 \begin{equation}
     \label{eq:minimum_L_l0}
     L_{\min}\geq \max_{\substack{\mathcal{T}\subseteq \mathbb{P}\\ |\mathcal{T}|=m}} 2 \sum_{p \in D_{\mathcal{T}}}\phi\left(p\right)\:.
\end{equation}

==> Background/Sparse_recovery/periodicity_compressive_sensing.tex <==
\subsection{Period estimation via sparse signal recovery} \label{subsec:period_estimation_sparse}
Given the model in \eqref{eq:NPD_model} it has been shown that a periodic signal admits a sparse representation in an NPD \cite{tenneti2015nested}. Therefore, sparse recovery methods such as BP have been employed to recover the sparse vector $\bx$, subsequently the underlying period of $\tilde{\by}$ based on the support set of $\bx$ \cite{vaidyanathan2014farey},\cite{tenneti2015nested}. In a preliminary version of this work \cite{saidi2021sparse}, we showed that the sufficient conditions in \eqref{eq:coherence_guarantee} and \eqref{eq:cumulative_coherence_guarantee} are of limited use when it comes to NPDs. Many of the existing conditions have been shown promise in the case of random dictionaries. However, for NPDs - deterministic and structured matrices - there is a gap between theory and practice. Our preliminary results in \cite{saidi2021sparse} were limited to a special case where $m = 1$, i.e., the periodic signal consists of one single period and in the absence of noise, where we established a tight bound that guarantee exact sparse recovery in NPDs. In this work, we extend our study to the more general case of periodic mixtures. We define new notions of coherence that leverage the structure of NPDs, and we establish new improved bounds that guarantee exact sparse recovery. In addition, we investigate the support recovery guarantees for the OMP algorithm in the presence of noise.


==> Contribution/Noise_free/ERC_NPD.tex <==
\subsection{Exact sparse recovery guarantees in the noise-free case}
\label{subsec:method_noiseless}
%\subsubsection{General case of periodic mixtures}
In this section, we establish exact recovery guarantees for periodic signals. Conditions such as \eqref{eq:coherence_guarantee} and \eqref{eq:cumulative_coherence_guarantee} ignore the structure of the NPDs, thus do not yield meaningful recovery bounds in this context, as will be shown in Section \ref{sec:result}. % shown of a sparse vector with sparsity level of interest.
% We will show in section \ref{sec:result} that conditions such as \eqref{eq:coherence_guarantee} and \eqref{eq:cumulative_coherence_guarantee} that  ignore the structure of the NPDs, do not yield meaningful guarantee for exact recovery of a sparse vector with sparsity level of interest. In this work, 
Therefore, we leverage the properties of NPDs, namely the Euler structure and the LCM property, to provide new and improved bounds tailored to NPDs. First, we assert the following result, which gives a sufficient condition for exact recovery for any periodic mixture.
%\input{Contribution/Noise_free/Theorem_mixture_general}
%\input{Contribution/Noise_free/Theorem_mixture_sparsity}
%\input{Contribution/Noise_free/Proof_mixture_theorem}
\input{Contribution/Noise_free/Theorem_mixture_period_estimation}

% \textcolor{blue}{The condition \eqref{} exploits our prior knowledge of }
For the special case where the periodic signal contains only one period, i.e., $m = 1$, we can assert the following result as a corollary of Theorem \ref{thr:mixture_general}.
\input{Contribution/Noise_free/corollary_single_period}


==> Contribution/Noise_free/Proof_mixture_theorem.tex <==
\begin{proof}
For a periodic mixture that consists of hidden periodic signals with periods $p_1,p_2,\ldots,p_m$, and from the LCM property of the NPDs we know that the periodic mixture can be decomposed using the atoms that belong to the divisors of the hidden periods. From Definition \ref{def:union_support_set}, set $D_\mathcal{T}$ contains all of the divisors of interest. Accounting for the Euler structure of the NPDs $S_\mathcal{T}$ is the index set of the atoms that belong to the divisors in $D_\mathcal{T}$. Without loss of generality, we assume that $S_\mathcal{T}$ is the exact support set of the mixture. Therefore, $\bK_{S_\mathcal{T}}$ is the NPD restricted to the support set of the mixture which has cardinality $|S_\mathcal{T}| = \sum_{d_i \in D_\mathcal{T}} \phi\left(d_i\right)$. Following from  \cite[Theorem 1]{tropp2004greed}, condition in \eqref{eq:ERC_mixture_sparse} is the sufficient condition to exactly recover the support set of $\tilde{\by}$ in \eqref{eq:NPD_model} under a NPD.
\end{proof}

==> Contribution/Noise_free/Theorem_mixture_sparsity.tex <==
\begin{theorem} \label{th:mixture_sparsity}
Suppose the matrix $\bK$ is a NPD of size $L\times N$, where $N = \sum_{p=1}^{P_\mathrm{max}} \phi\left(p\right)$. Let $\mathcal{T} \in \mathbb{Q}_k\left(m\right)$ and $S_{\mathcal{T}}$ be as in Definition \ref{def:union_support_set} with $k  = \sum_{d_i \in D_\mathcal{T}} \phi\left(d_i\right)$. If the following condition holds
\begin{equation}
    \label{eq:ERC_mixture_sparse}
    \begin{aligned}
        \|\left(\bK_{S_{\mathcal{T}}}^H\bK_{S_{\mathcal{T}}}\right)^{-1}\bK_{S_{\mathcal{T}}}^H\bK_{S_{\mathcal{T}}^c}\|_{1,1} <1
    \end{aligned}
\end{equation}
for all $\mathcal{T} \in \mathbb{Q}_k\left(m\right)$ then the BP in program \eqref{eq:l_1_norm} and OMP can exactly recover the support set of the sparse vector $\tilde{\bx}$ in \eqref{eq:NPD_model} for any periodic mixture of $m$ and sparsity level $k_m$ where its hidden periods are in $\mathbb{Q}_k\left(m\right)$.
\end{theorem}





==> Contribution/Noise_free/Theorem_mixture_sparsity_new.tex <==
\begin{corollary}
\label{cor:theorem_mixture_sparsity}
Assume $\by$ is a periodic mixture that consists of at most $m$ elements $p_1,\ldots,p_m$ and $\sum_{q \in D_{\{p_1,\ldots,p_m\}}} \phi\left(q\right) \leq k$. If \eqref{eq:ERC_mixture} holds for every $\mathcal{T} \in \mathbb{Q}_k\left(m\right)$, one can identify the hidden periods of the periodic mixture $\by$ via BP and OMP.
\end{corollary}


==> Contribution/Noise_free/Theorem_npd_upperbound_guarantee.tex <==
\begin{corollary}
\label{cor:guarantee_restrcited_coherence_npd}
Suppose $\bK$ is a NPD of size $L\times N$. Let $\zeta_p$ be the p-restricted inter coherence and $\nu_p$ the p-restricted intra-coherence of $\bK$ for period $p\in\mathbb{P}$  defined in \eqref{eq:restricted_inter_coh_special} and \eqref{eq:restricted_intra_coh_special}, respectively. Then, the condition in \eqref{eq:ERC_NPD} is satisfied if \eqref{eq:guarantee_restricted_coh_NPD} holds for all $p \in \mathbb{P}$.
\begin{equation}
    \label{eq:guarantee_restricted_coh_NPD}
    \begin{aligned}
        \zeta_p + \nu_p < 1 \:.
    \end{aligned}
\end{equation}
\end{corollary}


==> Contribution/Noise_free/Theorem_relaxed_per_set.tex <==
\begin{theorem}
\label{th:guarantee_restrcited_coherence_npd_strong}
Suppose that $\bK$ is an NPD, of size $L\times N$. For the ERC condition in (\ref{eq:ERC_NPD}) to hold, the following condition should satisfy for all $q$ in $\{1,\ldots,P_{max}\}$.
\begin{equation}
    \label{eq:guarantee_restricted_coh_NPD_strong}
    \zeta_I\left(k\right) + \zeta_1\left(k-1\right) < 1 \:.
\end{equation}
\end{theorem}
\begin{proof}
 \begin{equation*}
    \begin{aligned}
       \|\bK^{\dagger}_{S_p}\bK_{S_p^c}\|_1 \leq
       \|\left(\bK_{S_p}^H\bK_{S_p}\right)^{-1}\|_1\|\bK_{S_p}^H\bK_{S_p^c}\|_1 .
    \end{aligned}
\end{equation*}
 We can find upper bounds for the two factors of the RHS in the inequality. We begin with the second factor. It is easy to see that $\|\bK_{S_p}^H\bK_{S_p^c}\|_1\leq \zeta_I\left(k\right)$.
We follow the same reasoning of \cite{tropp2004greed} that used the Neumann series and Banach algebra to bound the first factor on the right hand side of the inequality. Since the dictionary $\bD$ is normalized we can write the following
\begin{equation*}
       \bK_{S_p}^H\bK_{S_p} = \bB + \bI_p,
\end{equation*}
subsequently we have
\begin{equation*}
       \|\bB\|_1 \leq \mu_1\left(k-1\right)
\end{equation*}
If $\nu_p<1$ we can write
\begin{equation*}
       \|\left(\bB + \bI_p\right)^{-1}\|_1 = \|\sum_{k=0}^\infty \left(-\bB\right)^k\|_1,
\end{equation*}
that is because the Neumman series $\sum_{k=0}^\infty \left(-\bB\right)^k$ converges to $\left(\bB + \bI_p\right)^{-1}$ \cite{tropp2004greed},\cite{kreyszig1978introductory}. Therefore, 
\begin{equation*}
    \begin{aligned}
       \|\left(\bK_{S_p}^H\bK_{S_p}\right)^{-1}\|_1 &= \|\sum_{k=0}^\infty \left(-\bB\right)^k\|_1\\
       &\leq \sum_{k=0}^\infty \|\bB\|^{k}_1\\
       &= \frac{1}{1-\|\bB\|^{k}_1} = \frac{1}{1-\mu_1\left(k\right)}.
    \end{aligned}
\end{equation*}
Hence,
\begin{equation}
\label{eq:proof_final_npd_l1_upperbound_inequality-strong}
 \|\bK^{\dagger}_{S_p}\bK_{S_p^c}\|_1 \leq \frac{\zeta_I\left(k\right)}{1-\mu_1\left(k\right)}.
\end{equation}
We conclude that if \eqref{} holds
\end{proof}


==> Contribution/Noise_free/Theorem_upperbound_single_sparse_level.tex <==
\textcolor{blue}{
\begin{corollary}
\label{cor:guarantee_single_sparselevel}
Suppose that $\bK$ is an NPD, of size $L\times N$. For a $p$-periodic signal with a $s$ sparse representation in the NPD, if the following condition satisfies
\begin{equation}
    \label{eq:guarantee_single_sparselevel}
    \zeta_p\left(s\right) + \nu_p\left(s-1\right) < 1 \:,
\end{equation}
then BP and OMP can recover the exact support of the periodic signal under the NPD, hence, the period $p$.
\end{corollary}
}


==> Contribution/Noise_free/corollary_single_period.tex <==
\begin{corollary}
\label{thr:ERC_npd_single}
Suppose the matrix $\bK$ is an NPD of size $L\times N$. Let $S_p$ be as in Definition \ref{def:union_support_set}.
% denotes the location of nonzero values in $\bx$, i.e., the support set of $\bx$ that corresponds to the $p$-periodic signal with $|S_p| = p$. 
If the following condition holds for every $p \in \mathbb{P}$,
\begin{equation}
    \label{eq:ERC_NPD}
    \begin{aligned}
        M_p := \|\left(\bK_{S_p}^H\bK_{S_p}\right)^{-1}\bK_{S_p}^H\bK_{S_p^c}\|_{1,1} <1
\end{aligned}
\end{equation}
then the BP program in \eqref{eq:l_1_norm} and the OMP algorithm can exactly recover the support set of the sparse vector $\bx$ in \eqref{eq:NPD_model}, and in turn, the period $p \in \mathbb{P}$.
\end{corollary}

==> Contribution/Noise_free/p_restricted_inter_coherence.tex <==
%\begin{definition}
%We define the nested subspace cumulative %inter-coherence as
%\label{def:p_restricted_inter_coherence}
\begin{equation}
    \label{eq:p_restrict_inter-coh}
    \zeta_p\left(s\right) \eqdef \max_{\Lambda_s\subseteq S_p}\max_{i \in \mathbb{N} \setminus S_p}\sum_{\substack{j \in \Lambda_s}} |\langle \bk_i,\bk_j\rangle|\:,
\end{equation}
%\end{definition}

==> Contribution/Noise_free/p_restricted_intra_coherence.tex <==
%\begin{definition}
%In addition we define the $p$-restricted cumulative intra-coherence 
%\label{def:p_restricted_intra_coherence}
\begin{equation}
    \label{eq:p_restrict_intra_coh}
    \nu_p\left(s\right) \eqdef \max_{\Lambda_s\subseteq S_p} \max_{i \in \Lambda_s} \sum_{\substack{j \in \Lambda_s\\i\neq j}} |\langle \bk_i,\bk_j\rangle|\:.
\end{equation}

%\end{definition}

==> Contribution/Noise_free/proof_npd_upperbound_guarantee.tex <==
\begin{proof}
Next we provide a sketch of the proof. We have
 \begin{equation*}
    \begin{aligned}
       \|\bK^{\dagger}_{S_p}\bK_{S_p^c}\|_1 &\leq
       \|\left(\bK_{S_p}^H\bK_{S_p}\right)^{-1}\|_1\|\bK_{S_p}^H\bK_{S_p^c}\|_1 
       \\       &=\|\left(\bK_{S_p}^H\bK_{S_p}\right)^{-1}\|_1 \zeta_p\:.
    \end{aligned}
\end{equation*}
Following the same reasoning in \cite{tropp2004greed}, we use the Neumann series and Banach algebra to bound the first factor on the right hand side of the above inequality. Since the dictionary $\bK$ is normalized, we can express the gram matrix as
\begin{equation*}
       \bK_{S_p}^H\bK_{S_p} = \bB + \bI_p
\end{equation*}
for some matrix $\bB$. Given the definition of the restricted intra-coherence in \eqref{eq:restricted_intra_coh_npd}, we have that
\begin{equation*}
       \|\bB\|_1 = \nu_p\:.
\end{equation*}
If $\nu_p<1$, then
\begin{equation*}
       \|\left(\bB + \bI_p\right)^{-1}\|_1 = \|\sum_{k=0}^\infty \left(-\bB\right)^k\|_1,
\end{equation*}
because the Neumman series $\sum_{k=0}^\infty \left(-\bB\right)^k$ converges to $\left(\bB + \bI_p\right)^{-1}$ \cite{tropp2004greed,kreyszig1978introductory}. Therefore, 
\begin{equation*}
    \begin{aligned}
       \|\left(\bK_{S_p}^H\bK_{S_p}\right)^{-1}\|_1 &= \|\sum_{k=0}^\infty \left(-\bB\right)^k\|_1\\
       &\leq \sum_{k=0}^\infty \|\bB\|^{k}_1\\
       &= \frac{1}{1-\|\bB\|_1} = \frac{1}{1-\nu_p}\:.
    \end{aligned}
\end{equation*}
Hence,
\begin{equation}
\label{eq:proof_final_npd_l1_upperbound_inequality}
 \|\bK^{\dagger}_{S_p}\bK_{S_p^c}\|_1 < \frac{\zeta_p}{1-\nu_p}\:.
\end{equation}
We conclude that if the RHS of (\ref{eq:proof_final_npd_l1_upperbound_inequality}) is less than 1 for all $p \in \mathbb{P}$, then the ERC in (\ref{eq:ERC_NPD}) holds.
\end{proof}




==> Contribution/Noise_omp/Noisy_omp_extra_removed_from_text.tex <==
\begin{equation}
B_{\infty}\left(\eta\right) = \{ \epsilon : \|\bX^T\epsilon\|_{\infty} \leq \sigma \sqrt{2 \left(1+\eta\right) \log p}\},
\end{equation}
where $\eta \geq 0$. 
\begin{lemma}
The Gaussian error $\epsilon \sim \mathcal{N}\left(\mathbf{0},\sigma^2\bI_n\right)$ satisfies
\begin{equation}
    P\left(\epsilon \in B_2\right) \geq 1 - \frac{1}{n}
\end{equation}
and
\begin{equation}
    P\left(\epsilon \in B_{\infty}\left(\eta\right)\right) \geq 1 - \frac{1}{2p^{\eta}\sqrt{\pi\log p}}.
\end{equation}
\end{lemma}
\begin{theorem}
Suppose $\epsilon \sim \mathcal{N}\left(\mathbf{0},\sigma^2\bI_n\right)$, $\mu < \frac{1}{2k-1}$ and all the nonzero coefficients $\beta_i$ satisfy
\begin{equation}
    |\beta_i| \geq \frac{2\sigma \sqrt{n + 2\sqrt{n \log n}}}{1-\left(2k-1\right)\mu}
\end{equation}
Then OMP with the stopping rule $\|r_i\|_{2}\leq \sigma \sqrt{n + 2\sqrt{n \log n}}$ selects exactly the correct subset $\bX\left(T\right)$ with probability at least $1-1/n$.
\end{theorem}
\begin{theorem}
Suppose $\epsilon \sim \mathcal{N}\left(\mathbf{0},\sigma^2\bI_n\right)$, $\mu < \frac{1}{2k-1}$ and all the nonzero coefficients $\beta_i$ satisfy
\begin{equation}
    |\beta_i| \geq \frac{2\sigma \sqrt{2\left(1+\eta\right)\log p}}{1-\left(2k-1\right)\mu}
\end{equation}
for some $\eta \geq 0$. Then OMP with the stopping rule $\|\bX'r_i\|_{\infty}\leq \sigma \sqrt{2\left(1+\eta\right)\log p}$ selects exactly the correct subset $\bX\left(T\right)$ with probability at least $1-k/p^{\eta}\sqrt{2\log p}$.
\end{theorem}

==> Contribution/Noise_omp/Theorem_noise_bounded.tex <==
\begin{theorem}
\label{thr:noise_bounded_general}
Suppose $\|\bw\|_2\leq \epsilon$, and $\by$ is a periodic mixture of $m$ periodic signals with its hidden period in $\mathcal{T}$ that has a sparse representation in an NPD. If \eqref{eq:ERC_mixture_sparse} holds, then the OMP algorithm with the stopping rule $\|\br_i\|_2\leq \epsilon$ recovers exactly the true support of $\by$ if all the nonzero coefficients $x_i$ satisfy the following:
\begin{equation}
    \label{eq:omp_npd_noise_bnd}
|x_i|\geq \frac{2\epsilon}{\left(1-M\right)\lambda_{\min}},
\end{equation}
where $M$ is the LHS of \eqref{eq:ERC_mixture_sparse} and  $\lambda_{\min}$ is the minimum eigenvalue of $\bK_{S_\mathcal{T}}^H\bK_{S_{\mathcal{T}}}$.
\end{theorem}

==> Contribution/Noise_omp/Theorem_noise_bounded_single.tex <==
\begin{corollary}
\label{thr:noise_bounded_single}
Suppose $\|\bw\|_2\leq \epsilon$, and $M_{\max} = \max_{p\in \mathbb{P}} M_p<1$. Then the OMP algorithm with the stopping rule $\|\br_i\|_2\leq \epsilon$ recovers exactly the true support of any $p$-periodic signal if all the nonzero coefficients $x_i$ satisfy the following:
\begin{equation}
    \label{eq:omp_noise_bnd_single}
|x_i|\geq \frac{2\epsilon}{\left(1-M_{\max}\right)\lambda^{\star}},
\end{equation}
where $\lambda^{\star} = \min_{p \in \mathbb{P}} \lambda_{\min}\left(p\right)$ and $\lambda_{\min}\left(p\right)$ is the minimum eigenvalue of $\bK_{S_p}^H\bK_{S_p}$.
\end{corollary}


%We can directly conclude the following:
%\begin{corollary}
%\label{cor:omp_bounded}

%\end{corollary}



==> Contribution/Noise_omp/Theorem_noise_bounded_weak.tex <==
\begin{theorem}
\label{thr:noise_omp_weak}
Suppose $\|\bw\|_2\leq \epsilon$ and for a sparsity level $k$, \eqref{eq:guarantee_single_sparselevel} holds. Then the OMP algorithm with the stopping rule $\|\br_i\|_2\leq \epsilon$ recovers the exact support of any $p$-periodic signal with sparsity level $k$ if all the nonzero coefficients $x_i$ satisfy the following:
\begin{equation}
    \label{eq:omp_npd_noise_sparse}
|x_i|\geq \frac{2\epsilon}{\left(1-\zeta_p\left(k\right) -\nu_p\left(k\right) \right)\lambda_{\min}\left(p\right)},
\end{equation}
\end{theorem}

==> Contribution/Noise_omp/Theorem_noise_bounded_weak_single.tex <==
\begin{theorem}
\label{thr:noise_omp_weak}
Suppose $\|\bw\|_2\leq \epsilon$ and for a sparsity level $s$, \eqref{eq:guarantee_single_sparselevel} holds. Then the OMP algorithm with the stopping rule $\|\br_i\|_2\leq \epsilon$ recovers the exact support of any $p$-periodic signal with sparsity level $k$ if all the nonzero coefficients $x_i$ satisfy the following:
\begin{equation}
    \label{eq:omp_npd_noise_sparse}
|x_i|\geq \frac{2\epsilon}{\left(1-\zeta_1\left(s\right) -\nu_1\left(s-1\right) \right)\lambda_{\min}\left(p\right)},
\end{equation}
\end{theorem}

==> Contribution/Noise_omp/Theorem_noise_gaussian.tex <==
\begin{theorem}
 \label{thr:noise_gaussian}
Suppose $\bw \sim \mathcal{N}\left(\mathbf{0},\sigma^2\bI_L\right)$, and $\by$ is a periodic mixture of $m$ periodic signals with its hidden periods in $\mathcal{T} \in \mathbb{Q}_k\left(m\right)$. % that has a sparse representation in an NPD supported on $S_{\mathcal{T}}$. 
If \eqref{eq:guarantee_NPD_strong} holds and all the nonzero coefficients $x_i$ satisfy
\begin{equation}
\label{eq:gaussian_coeff}
    |x_i| \geq \frac{2\sigma \sqrt{L + 2\sqrt{L\log L}}}{\left(1-\zeta_{k,m}-\nu_{k,m}\right)\left(1-\nu_{k,m}\right)}\:,
\end{equation}
then the OMP algorithm with the stopping rule $\|\br_i\|_{2}\leq \sigma \sqrt{L + 2\sqrt{L \log L}}$ recovers the exact support with probability at least $1-1/L$.
\end{theorem}


==> Contribution/lcm/lcm.tex <==
 Given an NPD, there exist a submatrix $\bC_p$ that spans the corresponding NPS $\mathcal{U}_p$, and in general $\mathcal{U}_{p_i} \not\perp \mathcal{U}_{p_j}$, when $i\neq j$. For the special case of the Ramanujan subspaces $\mathcal{S}_{p_i}\perp \mathcal{S}_{p_j}$. We leverage the orthogonality property of the Ramanujan subspaces and assert the following:
\begin{theorem}
\label{thr:lcm_npd}
Suppose the matrix $\bK$ is an NPD of size $L \times \sum_{p=1}^{P_{\max}}\phi\left(p\right)$, and $L_{\opt} = \lcm\left(1,2,\ldots,P_{\max}\right)$. Then BP can recover the exact support set of any periodic mixture.
\end{theorem}

\begin{remark}
From Theorem \ref{thr:lcm_npd}, we know that for $L = L_{\opt} =  \lcm\left(1,2,\ldots,P_{\max}\right)$ there is a unique representation for all periodic signals with periods in $\mathbb{P}$. Limiting the NPD, to the Farey and RPT dictionary allows the corresponding NPSs to enjoy the orthogonality as well, i.e., each of the submatrices $\bC_q$ will span the Ramanujan subspaces. For the RPT dictionary, we can specifically show that $\zeta_I\left(k\right) = 0$ and $\mu_I\left(k\right)<1$ and for the Farey dictionary $\zeta_I\left(k\right) = 0$ and $\mu_I\left(k\right) = 0$.
\end{remark}

%\begin{theorem}
%\label{thr:asymptotic_ramanujan}
%Suppose the matrix $\bK$ either the Farey or the RPT dictionary of size $L \times \sum_{p=1}^{P_{\max}}\phi\left(p\right)$, and $L - \lcm\left(1,2,\ldots,P_{\max}\right)<\delta$, where $\delta$ is a positive small constant. Then BP and OMP can recover the exact support set of any periodic mixture.
%\end{theorem}

%\begin{proof}
%From Theorem \ref{thr:asymptotic_npd}, we know that for $L = L_{\opt} =  \lcm\left(1,2,\ldots,P_{\max}\right)$ there is a unique representation for all periodic signals with periods in $\mathbb{P}$. For $L < L_{\opt}$, we should show that \eqref{eq:guarantee_restricted_coh_NPD_strong} holds.  Limiting the NPD, to the Farey and RPT dictionary allows the corresponding NPSs to enjoy the orthogonality as well, i.e., each of the submatrices $\bC_q$ will span the Ramanujan subspaces. However, it is apparent that the submatrices are not orthogonal with any arbitrary $L$. However, when the between $L$ and $L_{\opt}$ is small enough, all the  submatrices start to get closer to their complete periodic cycle, and the inner product between the atoms that belong to different submatrices goes to $0$, i.e.,
%$\bC_{p_i}^H\bC_{p_j} \rightarrow 0$ for $i\neq j$ when $L-L_{\opt} < \delta$ and $L\rightarrow L_{\opt}$. Therefore, following the Definition \ref{def:cumulative_inter_coh}, $\zeta_I\left(k\right) \rightarrow \epsilon$ as it accounts for inter coherence between different submatrices. 


%\end{proof}



==> Introduction/periodicity_thorugh_dictionaries.tex <==
In \cite{tenneti2015nested} authors introduced a new family of matrices called nested periodic dictionaries (NPDs) and showed that periodic signals may admit sparse representation under NPDs. Therefore, one can model a periodic signal of length $L$ in the matrix form as
\begin{equation}
    \label{eq:NPD_model_noisy}
    \begin{aligned}
    \by = \bK\bx +\bw
    \end{aligned},
\end{equation}
where $\bK \in \mathbb{C}^{L\times N}$ is the NPD, $\bw \in \mathbb{R}^L$ is the noise vector, $\by$ is a vector of length $L$ that contains the periodic entries in addition to noise, and $\bx \in \mathbb{C}^{N}$ is its sparse representation.
Although introduced recently, some real-world applications of NPDs have been explored. For instance, in \cite{saidi2019detection}, authors developed a new framework to detect SSVEPs using Ramanujan periodicity transform (RPT) dictionary that is an example of NPDs. In  \cite{tenneti2016detecting}, NPDs were used to detect tandem repeats in DNA and  in \cite{mathur2021ramanujan} a method based on Ramanujan subspaces is proposed for classification of epileptic EEG signals. In \cite{tenneti2015nested,tenneti2016unified,vaidyanathan2014farey}, authors proposed different algorithms to estimate the hidden periods in a periodic mixture using NPDs. As discussed in these works one can estimate the hidden periods by recovering the support set of $\bx$, i.e., the location of the non-zero entries in $\bx$. However, under an underdetermined system of equations - when the number of measurements (rows) $L$ is smaller than the number of atoms (columns) $N$-  a sparse recovery framework can identify the support set from (\ref{eq:NPD_model_noisy}) \cite{tenneti2018minimum,vaidyanathan2014farey}. It has been shown through numerical simulations that sparse recovery techniques can recover the support set of the sparse vector that represent a periodic sequence in \eqref{eq:NPD_model_noisy} \cite{vaidyanathan2014farey},\cite{tenneti2015nested}. However, the performance of such techniques depend on the family of functions that have been employed to construct the NPD. Also, there is no evidence if these techniques recover the exact support. On the contrary, numerical simulation shows that the recovered support set may be contained in a larger set, and it might be needed to force some coefficients to zero if they are very small in the recovered $\bx$. We refer to this process as thresholding. On the other hand, the existing recovery guarantees stand short when the dictionary is an NPD - a deterministic and structured dictionary.  To fill the gap between theory and practice, we investigated the existence of support recovery guarantees for NPDs, for the noise-free scenario where the model in \eqref{eq:NPD_model_noisy} reduces to 
\begin{equation}
    \label{eq:NPD_model}
    \begin{aligned}
    \tilde{\by} = \bK\bx
    \end{aligned},
\end{equation}
where $\tilde{\by}$ is the noise-free periodic vector and $\tilde{\bx}$ is its sparse representation. We derived our preliminary results for a special case where the periodic signal is consisted of a single period \cite{saidi2021sparse}. In this study, we extend our work to the periodic mixtures where $m$ periodic signals construct the observation vector $\by$. Furthermore, we consider the model in \eqref{eq:NPD_model_noisy} where the periodic observations are in the presence of noise.

==> Results/sampling.tex <==
\subsection{Non-uniform sampling of the measurements} \label{subsec:results_sampling}
There has been some efforts to investigate sparse recovery guarantees when the measurements are selected randomly \cite{candes2006robust,candes2007sparsity}. 
In the period estimation problem, we assumed that we have access to consecutive measurements of the periodic signal. These studies inspired us to investigate a non-uniform sampling framework, and evaluate the established guarantees for such a scenario.
As discussed in section \ref{subsec:NPM}, NPMs are $P \times P$ matrices, that contain sub-matrices $\bC_q$, where $q|P$. One drawback of the NPMs is that their ability to estimate the hidden periods of a mixture is limited to the divisors of $P$, as opposed to the NPDs that span the nested period subspaces of all values between $1$ to $P_{\max}$. In this section, we consider a case where $P = \lcm\left(p_1,p_2,...,p_{m}\right)$ that gives rise to a NPM that is able to capture hidden periods of interest.
In this section we compare the established guarantee in \eqref{eq:guarantee_NPD_strong}, for two different scenarios. 1) The rows of the dictionary are randomly selected from the NPM. 2) The rows of the dictionary are selected consecutively from the NPM. In both cases the number of selected rows is equal to $L$. We employ two of the NPMs, that span the Ramanujan subspaces, the DFT-based NPM and the RPT. We consider a case where $\mathbb{P}^{\star} = \{1,2,3,4,5,6,7,8,9,10,12,14,15,16,18,20\}$. The LCM of the values is $P = 5040$. 
\input{figures_tex/Sampling/sampling_90}
Fig. \ref{fig:sampled90} shows the result for the DFT-based dictionary and the RPT-based dictionary when the rows are sampled at $90\%$. As illustrated, the random sampling of the DFT-based matrix, has improved the bound significantly and show that exact recovery guarantee exist for sparse vectors with sparsity level $40$, as opposed to the consecutive sampling where the sparsity level of achievable guarantee is $5$. On the side, such improvement has not been observed for the RPT dictionary.



==> Results/tables_block_coherence.tex <==
%\begin{table}
%    \caption{Coherence values for different NPDs, while $L = 128$}
%    \label{tab:npd_coherence}
%    \centering
%    \begin{tabular}{c|c|c|c} 
%         NP Dictionaries&Standard coherence& Block coherence& Sub coherence\\\hline
%         DFT&&&\\\hline
%         Ramanujan&0.5836&0.1171&0.5836
%    \end{tabular}
%\end{table*}
\begin{table}
    \caption{Standard coherence values for different NPDs, with $P_\mathrm{max} = 100$ and $L = 2885$.}
    \label{tab:npd_coherence_L_new}
    \centering
    \begin{tabular}{c|c|c} 
         NPD & Standard coherence & RHS of the condition in (\ref{eq:coherence_guarantee}) \\\hline
         Farey&0.8660&1.0773\\\hline
         RPT&0.5070&1.4862
    \end{tabular}
\end{table}

==> figures_tex/ERC_single/Figure_9_single_ERC.tex <==
\begin{figure}
    \centering
        \includegraphics[width = \linewidth,height = 8cm]{Figures/ERC_single/Figure_9.eps}
    \caption{Evaluation of the ERC in \eqref{eq:ERC_NPD} (a) for the Farey, RPT and natural NPD when $P_{\max} = 100$ and $L = 1915$. A comparison between the ERC in \eqref{eq:ERC_NPD} with respect to $L$ for (b) The Farey dictionary (c) RPT and (d) natural NPDs.}
    \label{fig:ERC_single}
\end{figure}

==> figures_tex/ERC_single/guarantee_single_ERC.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 3.5cm]{Figures/ERC_single/guarantee_single_ERC.eps}
        \caption{}
        \label{subfig:ERC_single_1915}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 3.5cm]{Figures/ERC_single/Farey_single_ERC.eps}
    \caption{}
    \label{subfig:ERC_single_Farey}
    \end{subfigure}
    
   \begin{subfigure}[b]{0.23\textwidth}
   \centering
    \includegraphics[width = \textwidth,height = 3.5cm]{Figures/ERC_single/RPT_single_ERC.eps}
    \caption{}
    \label{subfig:ERC_single_rpt}
   \end{subfigure}
   \hfill
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width = \textwidth,height = 3.5cm]{Figures/ERC_single/natural_single_ERC.eps}
    \caption{}
    \label{subfig:ERC_single_natural}
    \end{subfigure}

    \caption{Evaluation of the condition in \eqref{eq:ERC_NPD} (a) for the Farey, RPT and natural NPD when $P_{\max} = 100$ and $L = 1915$. A comparison between the ERC in \eqref{eq:ERC_NPD} with respect to $L$ for (b) The Farey dictionary (c) RPT and (d) natural NPDs.}
    \label{fig:ERC_single}
\end{figure}

==> figures_tex/ERC_single/phase_transition.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.22\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 3cm]{Figures/phase_transition/dft_P100_L2800.eps}
        \caption{}
        \label{subfig:[pt_farey}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.22\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 3cm]{Figures/phase_transition/RPT_P100_L2800.eps}
    \caption{}
    \label{subfig:pt_rpt}
    \end{subfigure}
    
   \begin{subfigure}[b]{0.22\textwidth}
   \centering
    \includegraphics[width = \textwidth,height = 3cm]{Figures/phase_transition/Natural_P100_L2800.eps}
    \caption{}
    \label{subfig:pt_natural}
   \end{subfigure}
   \hfill
    \begin{subfigure}[b]{0.22\textwidth}
    \centering
    \includegraphics[width = \textwidth,height = 3cm]{Figures/phase_transition/random_P100_L2800.eps}
    \caption{}
    \label{subfig:pt_random}
    \end{subfigure}
    \caption{Phase transition plots that show the achievability of the bound in \eqref{eq:guarantee_single_sparselevel} when $P_{\max} = 100$ and $L = 2875$ for (a) the Farey (b) the RPT (c) the natural and (d) the random NPD. The yellow color shows where the condition holds, and the dark color shows when the condition is short to guarantee exact recovery.}
    \label{fig:pt}
\end{figure}

==> figures_tex/ERC_single/upperbounds.tex <==
\begin{figure*}
\begin{subfigure}[b]{0.33\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 4cm]{Figures/Guarantees_NPD_ERC/cumulative_coh_all_L_2885.eps}
        \caption{}
        \label{subfig:standard_cumulative_Farey}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 4cm]{Figures/Guarantees_NPD_ERC/upperbounds/upperbound_P100_L_1915.eps}
        \caption{}
        \label{subfig:upperbound_P100_L_1915}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 4cm]{Figures/Guarantees_NPD_ERC/upperbounds/upperbound_P100_L_2875.eps}
    \caption{}
    \label{subfig:upperbound_P100_L_2875}
    \end{subfigure}
    %\begin{subfigure}[b]{0.33\textwidth}
    %\centering
    %    \includegraphics[width = \textwidth,height = 6cm]{Figures/Guarantees_NPD_ERC/upperbounds/upperbound_P100_L_2885.eps}
    %\caption{}
    %\label{subfig:upperbound_P100_L2885}
    %\end{subfigure}
    \caption{(a) The condition \eqref{eq:cumulative_coherence_guarantee} based on the cumulative coherence \cite{tropp2004greed} for the Farey and RPT dictionary for $P_\mathrm{max}= 100$ and $L = 2885$.  Conditions in (\ref{eq:ERC_NPD}) and (\ref{eq:guarantee_restricted_coh_NPD}) for the Farey dictionary (b) for $P_{\max}= 100$  and $L = 1915$, and (c) $L = 2875$.}
    \label{fig:upperbound_Farey_P100}
\end{figure*}

==> figures_tex/Noise_result/noise_bounded_dft.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 4cm]{Figures/Noise/mse_DFT.eps}
        \caption{}
        \label{subfig:noise_bounded_dft_mse}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 4cm]{Figures/Noise/average_count.eps}
    \caption{}
    \label{subfig:noise_bounded_dft_avg}
    \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 4cm]{Figures/Noise/MSE_L1000_P60_DFT.eps}
        \caption{}
        \label{subfig:noise_bounded_dft_mse_all}
    \end{subfigure}
    \caption{(a) MSE and (b) average error count for the OMP algorithm, in the presence of the $\ell_2$-norm bounded noise. The nonzero coefficients are greater than the threshold value. (c) MSE for the OMP, when the conditions in Theorem \ref{thr:noise_bounded_single} are satisfied. Here, $P_{\max} = 60$ and $L = 1000$ and the Farey dictionary is used.}
    \label{fig:noise_bounded_dft}
    
\end{figure*}

==> figures_tex/Noise_result/noise_bounded_rpt.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 4cm]{Figures/Noise/ERC_1.eps}
        \caption{}
        \label{subfig:noise_bounded_rpt_erc}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 4cm]{Figures/Noise/RPT_P20_L100_8.eps}
    \caption{}
    \label{subfig:noise_bounded_rpt_rmse}
    \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 4cm]{Figures/Noise/success_rate_p20_L100_8.eps}
        \caption{}
        \label{subfig:noise_bounded_rpt_success}
    \end{subfigure}
    \caption{(a) $M_k\left(1\right)$, (b) RMSE, and (c) the success rate for the OMP algorithm, in the presence of the $\ell_2$-norm bounded noise. The nonzero coefficients are greater than the threshold value. Here, $P_{\max} = 20$ and $L = 100$ and the RPT dictionary is used.}
    \label{fig:noise_bounded_rpt}
    
\end{figure*}

==> figures_tex/Noise_result/noise_gaussian.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 3.5cm]{Figures/Noise/Gaussian/success_rate_alpha.eps}
        \caption{}
        \label{subfig:noise_gaussian_successrate}
    \end{subfigure}
    \hfill
     \begin{subfigure}[b]{0.23\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 3.5cm]{Figures/Noise/Gaussian/rmse.eps}
        \caption{}
        \label{subfig:noise_gaussian_rmse}
    \end{subfigure}
    \caption{(a) Success rate and (b) RMSE for OMP.}
    \label{fig:noise_gaussian}
    
\end{figure}

==> figures_tex/Sampling/sampling_90.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 3cm]{Figures/Sampling/upper_bound_strong_dft_90.eps}
        \caption{}
        \label{subfig:upperbound_sampled_dft}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 3cm]{Figures/Sampling/upper_bound_strong_rpt_90.eps}
    \caption{}
    \label{subfig:upperbound_sampled_rpt}
    \end{subfigure}
    \caption{Two versions of NPD is constructed by sampling rows from a) the DFT-based NPM and b) RPT-based NPM. The sampling is managed i) randomly with sampling rate of $90 \%$ and ii) consecutively.  $\mathbb{P}^{\star}$ is as described in section \ref{subsec:results_sampling}}
    \label{fig:sampled90}
\end{figure}



==> figures_tex/cumulative_example/coherence_example.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 6cm]{Figures/example/coherence_1.png}
        \caption{}
        \label{subfig:coherence_ex_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
\includegraphics[width = \textwidth,height = 6cm]{Figures/example/coherence_2.png}
    \caption{}
    \label{subfig:coherence_ex_2}
    \end{subfigure}
    \caption{Not finished}
    \label{fig:coherence_ex}
\end{figure*}

==> figures_tex/cumulative_example/coherence_example2.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 4cm]{Figures/example/coherence_4.png}
        \caption{}
        \label{subfig:coherence_ex2_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
\includegraphics[width = \textwidth,height = 4cm]{Figures/example/coherence_5.png}
    \caption{}
    \label{subfig:coherence_ex2_2}
    \end{subfigure}
        \begin{subfigure}[b]{0.32\textwidth}
    \centering
\includegraphics[width = \textwidth,height = 4cm]{Figures/example/coherence_3.png}
    \caption{}
    \label{subfig:coherence_ex2_3}
    \end{subfigure}
    \caption{Calculation of the NPI in \eqref{eq:npi_coherence}. (a) For $\mathcal{T} = \{2,5\} \in \mathbb{Q}_6\left(2\right)$, the absolute value of the the inner products of the atoms in $S_\mathcal{T}$ and $S_\mathcal{T}^c$ are shown in green color. The red ellipses mark the summands (inner products) % values that need to be added 
    in the summation over $j\in S_{\mathcal{T}}$ \textcolor{blue}{for $i = 5$}. (b) The same is shown for $\mathcal{T} = \{3,4\} \in \mathbb{Q}_6\left(2\right)$. The NPI is obtained as the maximum of all summations among all members of $\mathbb{Q}_6\left(2\right)$.
    % by maximizing over the maximum summations from all members of $\mathbb{Q}_6\left(2\right)$. 
    (c) The difference between the NPI and NPI-CC, for $\mathcal{T} = \{3,4\}$ and $s = 3$, instead of summing over all $j \in S_{\mathcal{T}}$ we sum over the largest $s$ values.}
    \label{fig:coherence_ex2}
\end{figure*}

==> figures_tex/cumulative_example/coherence_example3.tex <==
\begin{figure*}
    \centering
        \includegraphics[width = \textwidth,height = 4cm]{Figures/example/Coherence_ex3.eps}
    \caption{Calculation of the NPI in \eqref{eq:npi_coherence}. (a) For $\mathcal{T} = \{2,5\} \in \mathbb{Q}_6\left(2\right)$, the absolute value of the inner products of the atoms in $S_\mathcal{T}$ and $S_\mathcal{T}^c$ are shown in green color. The red ellipses mark the summands (inner products) % values that need to be added 
    in the summation over $j\in S_{\mathcal{T}}$ for $i = 3$. (b) The same is shown for $\mathcal{T} = \{3,4\} \in \mathbb{Q}_6\left(2\right)$. The NPI is obtained as the maximum of all summations among all members of $\mathbb{Q}_6\left(2\right)$.
    % by maximizing over the maximum summations from all members of $\mathbb{Q}_6\left(2\right)$. 
    (c) The difference between the NPI and CNPI, for $\mathcal{T} = \{3,4\}$ and $s = 3$, instead of summing over all $j \in S_{\mathcal{T}}$ we sum over the largest $s$ values.}
    \label{fig:coherence_ex2}
\end{figure*}

==> figures_tex/cumulative_example/coherence_example5.tex <==
\begin{figure*}
    \centering
        \includegraphics[width = \textwidth,height = 5cm]{Figures/example/Coherence_ex1.eps}
    \caption{Calculation of the NPI in \eqref{eq:npi_coherence}. (a) For $\mathcal{T} = \{3,4\} \in \mathbb{Q}_6\left(2\right)$. The atoms in $S^c_{\mathcal{T}}$ are shown in green boxes and atoms in $S_{\mathcal{T}}$ are shown in blue boxes. The inner summation in \eqref{eq:npi_coherence} computes the summation over the absolute value of the inner products between one atom from $S^c_{\mathcal{T}}$, - for example $i = 7$ marked with a red rectangle -  and all the atoms in $S_{\mathcal{T}}$. (b) The inner products of the atoms in $S_\mathcal{T}$ and $S_\mathcal{T}^c$ are shown in green color. The red ellipse mark the summands (inner products) in the summation over $j\in S_{\mathcal{T}}$ for $i = 7$, and the result is shown in yellow color.
    (c) The difference between the NPI and CNPI, for $\mathcal{T} = \{3,4\}$ and $s = 3$, instead of summing over all $j \in S_{\mathcal{T}}$ we sum over the largest $s$ values.}
    \label{fig:coherence_ex2}
\end{figure*}

==> figures_tex/mixture/old/mixture_erc_m1_m2.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.22\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 3cm]{Figures/mixture/Farey_direct_and_up_1915.eps}
        \caption{}
        \label{subfig:farey_mixture_bounds}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.22\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 3cm]{Figures/mixture/Farey_bounds_new_old.eps}
    \caption{}
    \label{subfig:farey_mixture_bounds_old}
    \end{subfigure}
    
   \begin{subfigure}[b]{0.22\textwidth}
   \centering
    \includegraphics[width = \textwidth,height = 3cm]{Figures/mixture/RPT_direct_and_up_2875.eps}
    \caption{}
    \label{subfig:rpt_mixture_bounds}
   \end{subfigure}
   \hfill
    \begin{subfigure}[b]{0.22\textwidth}
    \centering
    \includegraphics[width = \textwidth,height = 3cm]{Figures/mixture/RPT_new_old_2875.eps}
    \caption{}
    \label{subfig:rpt_mixture_bounds_old}
    \end{subfigure}
    \caption{Phase transition plots that show the achievability of the bound in \eqref{eq:guarantee_single_sparselevel} when $P_{\max} = 100$ and $L = 2875$ for (a) the Farey (b) the RPT (c) the natural and (d) the random NPD. The yellow color shows where the condition holds, and the dark color shows when the condition is short to guarantee exact recovery.}
    \label{fig:mixture_bounds}
\end{figure}

==> figures_tex/mixture/old/mixture_erc_m1_m2_2.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 6cm]{Figures/mixture/Farey_direct_and_up_old_1915.eps}
        \caption{}
        \label{subfig:dft_mixture_bounds_all}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 6cm]{Figures/mixture/RPT_direct_and_up_old_2875_nl.eps}
    \caption{}
    \label{subfig:rpt_mixture_bounds_all}
    \end{subfigure}
    \caption{achievability of the conditions in (\ref{eq:ERC_mixture_sparse}) and \eqref{eq:guarantee_NPD_strong} and a comparison to \eqref{eq:cumulative_coherence_guarantee} for (a) the Farey dictionary when $L = 1915$ and (b) the RPT dictionary when $L = 2875.$}
    \label{fig:mixture_bounds_all}
\end{figure*}

==> figures_tex/mixture/old/mixture_erc_m2_old.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 6cm]{Figures/mixture/mixture_old/mixture_ERC_vs_sparsity_all_dft_old.eps}
        \caption{}
        \label{subfig:ERC_mixture_2_dft}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 6cm]{Figures/mixture/mixture_old/mixture_ERC_vs_sparsity_all_rpt_old.eps}
    \caption{}
    \label{subfig:ERC_mixture_2_rpt}
    \end{subfigure}
    \caption{Evaluation of the ERC condition in (\ref{eq:ERC_mixture_sparse}) for (a) the Farey dictionary when $L = 1915$ and (b) the RPT dictionary when $L = 2875.$}
    \label{fig:ERC_mixture_direct}
\end{figure*}

==> figures_tex/mixture/old/mixture_upperbound.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 4cm]{Figures/mixture/upper_bound/Farey_L2875.eps}
        \caption{}
        \label{subfig:mixture_upperbound_farey}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 4cm]{Figures/mixture/upper_bound/RPT_L2875.eps}
    \caption{}
    \label{subfig:mixture_upperbound_rpt}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 4cm]{Figures/mixture/upper_bound/natural_L2875.eps}
    \caption{}
    \label{subfig:mixture_upperbound_natural}
    \end{subfigure}
    \caption{A comparison between the upper bound in \eqref{eq:cumulative_coherence_guarantee} and the newly derived bound in \eqref{eq:guarantee_NPD_strong} for (a) the Farey (b) RPT and (c) natural dictionaries when $P_{\max = 100}$ and $L = 2875$.}
    \label{fig:strong_upperbound}
\end{figure*}

==> figures_tex/numerical_BP_ITW/numerical_BP.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 6cm]{Figures/numerical_results_BP/success_rate_P100_Farey_all.eps}
        \caption{}
        \label{subfig:BP_P100_L_200}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 6cm]{Figures/numerical_results_BP/success_rate_P100_RPT_all.eps}
    \caption{}
    \label{subfig:BP_P100_L_400}
    \end{subfigure}
    \caption{The average Success rate when recovering the sparse vectors using BP. Here $P_{\max}= 100$. (a) With the Farey dictionary and $L = 2P_{\max}=200$, (b) $L = 500$. With the RPT dictionary when (c) $L= 500$ and (d) $L = 800$.}
    \label{fig:BP_P_100}
\end{figure*}

==> figures_tex/numerical_BP_ITW/numerical_BP_all.tex <==
\begin{figure}
    \centering
    \centering
        \includegraphics[width = \linewidth,height = 6cm]{Figures/numerical_results_BP/success_rate_P100_all_new.eps}
    \caption{The average success rate for recovering the sparse vectors using BP. Here, $P_\mathrm{max}=100$. For the Farey dictionary, $L =200$ and $L = 500$. For the RPT dictionary $L= 500$.}
    \label{fig:BP_P100_all}
\end{figure}

==> figures_tex/numerical_BP_ITW/recovery_sample.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 3cm]{Figures/recovery_samples/L_1915_all_indices.eps}
        \caption{}
        \label{subfig:recovery_sample_all}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
        \includegraphics[width = \textwidth,height = 3cm]{Figures/recovery_samples/L_1915_vs_oracle.eps}
    \caption{}
    \label{subfig:recovery_sample_vs_oracle}
    \end{subfigure}
    \caption{}
    \label{fig:recovery_sample}
\end{figure}
